Uncertainty quantification for distributed regression

The ever-growing size of the datasets renders well-studied learning techniques, such as Kernel Ridge Regression, inapplicable, posing a serious computational challenge. Divide-and-conquer is a common remedy, suggesting to split the dataset into disjoint partitions, obtain the local estimates and average them, it allows to scale-up an otherwise ineffective base approach. In the current study we suggest a fully data-driven approach to quantify uncertainty of the averaged estimator. Namely, we construct simultaneous element-wise confidence bands for the predictions yielded by the averaged estimator on a given deterministic prediction set. The novel approach features rigorous theoretical guaranties for a wide class of base learners with Kernel Ridge regression being a special case. As a by-product of our analysis we also obtain a sup-norm consistency result for the divide-and-conquer Kernel Ridge Regression. The simulation study supports the theoretical findings.

==> generalproofs.tex <==
%!TEX root = main.tex
\section{General proofs}

==> setting.tex <==
%!TEX root = main.tex
\section{Theoretical analysis}
\subsection{Assumptions}
First of all, we impose a polynomial rate of decay on the eigenvalues of $\kdd$.
\begin{assumption}[Polynomial eigendecay]\label{polyeigen}
  Let there exist a constant $b>1$ s.t. for  the $j$-th largest eigenvalue $\mu_j$ of $\kdd$
  \begin{equation}
    \mu_j \asymp j^{-b}.
  \end{equation}
\end{assumption}
As demonstrated in \citep{Yang2017},  \ref{polyeigen} holds for \matern~kernel with smoothness $\alpha$ in a $d$-dimensional space with $b=2\alpha+d$. Another popular example is a Squared Exponential kernel, which is known to exhibit an exponential rate of eigendecay. With some abuse of formality, our results can be applied in this case with $b=\infty$. Alternatively, the argument can be carefully repeated with minimal augmentation in this case as well.

We assume the eigenfunctions of the kernel to be bounded. 
The analysis in \citep{Yang2017a,Bhattacharya2017} proves the assumption holds for \matern~kernel under uniform and normal distributions of covariates on a compact.
\begin{assumption}[Boundness of eigenfunctions]\label{eigenbound}
  Denote a normalized eigenfunction corresponding to the $j$-th largest eigenvalue as $\phi_j(\cdot)$.
  Let there exist a positive constant $\phiinf$ s.t. \linebreak $\sup_j\max_{X\in\X} \abs{\phi_j(X)} \le \phiinf $.
\end{assumption}
Now consider an integral operator
\begin{equation}
  L_k(f) = \int_X k(X, \cdot) f(X) d \pi
\end{equation}
and denote {\it effective dimension} as
\begin{equation}
  \trace \coloneqq \tr{{\inv{\brac{L_k + \rho I}}L_k}}.
\end{equation}
Further, we impose Hölder-type source condition \cite{Mucke2018,lin2017distributed}
\begin{assumption}\label{rass}
  Let there exist $r\in (1/2,1]$ and $h \in \Ltwo$ s.t. 
  \begin{equation}
    \fstar = L_k^r(h). 
  \end{equation}
\end{assumption}

In conclusion we impose sub-Gaussianity assumption over noise, that being a common relaxation of Gaussianity.
\begin{assumption}[Sub-Gaussianity]\label{subgaussass}
  Let there exist a constant $\g^2$ s.t. for all $a\in \R$
  \begin{equation}
    \E{\exp(a\varepsilon_1)s} \le \exp\brac{\frac{\g^2a^2}{2}}.
  \end{equation}
\end{assumption}
